Safe-FCL: Continual Risk Awareness and Fine-Grained Safety Aggregation for Federated Continual Learning of LLMs

Federated fine-tuning enables large language models (LLMs) to learn collaboratively from distributed client data, but malicious client updates can compromise global model safety. As federated tasks evolve, changing malicious update patterns challenge the ability of existing defenses to maintain reliable risk detection over time. To address this challenge, we propose Safe-FCL, a framework integrating continual risk awareness with fine-grained safety aggregation for federated continual learning of LLMs. Specifically, the Continual Risk Awareness (CRA) mechanism learns emerging risk patterns across sequential tasks and constrains detector updates using a protective subspace derived from historical features, mitigating forgetting of previously learned malicious patterns while adapting to new risks. To translate risk awareness into aggregation-level safety control, the Fine-Grained Safety Aggregation (FGSA) mechanism combines client-level risk assessments from CRA with module-level deviations from historical update behavior to adaptively regulate aggregation contributions, suppressing potentially malicious updates while minimizing unnecessary restrictions on benign updates. Extensive experiments demonstrate that Safe-FCL outperforms current SOTA methods, improving global-model Rule and MD-Judge scores in federated continual learning by 0.41% and 0.64%, respectively, while increasing average risk recognition accuracy by 2.01%.

==> Safe-FCL_Experiments_revised.tex <==
% Revised Experiments text for Safe-FCL.
% This file contains NO table environments. It cites the three tables
% already present in the user's manuscript. Do not paste duplicate tables.
%
% Existing labels:
% tab:updated_rule_mdjudge  -- global-model safety, Rule/MD-Judge
% tab:safe_fcl_comparison   -- continual probe AA/AF/New ACC/Task 5
% tab:ablation_avg_t1_t4  -- safety ablation
%
% Before submission: confirm the task order associated with these tables,
% independent-run statistics, evaluation configuration, and signed AF
% definition. The current dataset manifest is exploratory, not final-audited.

\section{Experiments}
\label{sec:experiments}

We evaluate Safe-FCL along two complementary dimensions: global-model safety across sequential tasks and the continual risk-recognition ability of the detector. We also examine the contributions of CRA and FGSA using the available component comparisons. The reported safety and continual-probe tables cover the first four learning stages; the additional fifth-task results are discussed only where available.

\subsection{Experimental Setup}
\label{sec:experimental_setup}

\noindent\textbf{Tasks and Data.}
The evaluation involves five successive safety-related domains, spanning digital security, privacy protection, fraud and deception, physical and public safety, and discrimination-related harms. The existing tables report four sequential learning stages, with an additional fifth stage for evaluating transfer of an unchanged risk detector to a new task domain. According to the current data manifest, each task has 5,000 model-training examples (3,500 benign and 1,500 harmful), 714 validation examples, 1,429 evaluation examples, and a separate pool of 2,810 texts for constructing probe updates. The main text and tables refer to learning stages rather than assuming that stage indices always coincide with original task identifiers.
% TODO: Explicitly identify the task order underlying each reported table.
% The recorded protocols include T1-T2-T3-T4-T5 and T3-T1-T4-T2-T5.
% Confirm dataset audit/release status before claiming final verified splits.

\noindent\textbf{Federated Training.}
Experiments use Llama-3.1-8B with an 8-bit frozen backbone and trainable LoRA adapters on the query and value projections. LoRA uses rank 8, scaling parameter 16, and dropout 0.05. The federation contains ten clients, including seven benign and three malicious clients. Three clients participate per communication round, and each task runs for 100 rounds. Each selected client trains on 160 sampled local examples for ten optimizer steps, using an effective batch size of 16. The main local learning rate follows a task-wise cosine schedule from $5\times10^{-5}$ to $10^{-6}$. Global LoRA parameters are inherited between tasks. The risk-assessment trajectory uses the same selected local examples but starts from a fixed task-initial reference and uses a constant learning rate of $5\times10^{-5}$; it is not used for model aggregation.
% TODO: Report sequence length for the result set being presented; recorded
% task-order configurations use different limits (512 versus 1024).

\noindent\textbf{Risk Detector and Aggregation.}
For each of the first four stages, CRA collects 300 labeled stepwise update features (10 collection rounds, three clients per round, and ten local steps per client). The probe receives jointly $L_2$-normalized changes in selected first-layer LoRA-B parameters and uses a two-layer classifier with a 64-dimensional hidden layer. Labeled features are split into 270 training and 30 validation updates; this split is made at the update level, not the client or trajectory level. The probe is fitted with class-weighted binary cross-entropy and constrained candidate parameter updates, then held fixed during the stage's federated rounds. At the fifth stage, the detector from Stage 4 is reused without further adaptation, while global-model training and FGSA statistical updates continue. FGSA uses risk scores and the magnitude and directional deviations of actual local LoRA updates to gate module contributions. The risk classification threshold, suppression exponent, round-skipping threshold, module gating strength, and historical-statistics update rate are $0.8$, $7$, $0.2$, $1$, and $0.1$, respectively.

\noindent\textbf{Baselines and Metrics.}
For global-model safety, comparisons include FedAvg, FLAME, LASA, and the Step-, Client-, and Shadow-Level variants of Safe-FedLLM. We report Rule and MD-Judge scores, where higher values indicate safer generated responses. Each stage's average is the arithmetic mean over tasks learned up to that stage. Continual risk-recognition performance is assessed separately using average accuracy (AA), average forgetting (AF), and new-task accuracy (New ACC). The signed AF values are retained as reported, including small negative values. Additional fifth-task probe accuracies are incomplete and are not included in the four-stage averages.
% TODO: Specify the exact signed AF reference definition, task-order mapping,
% evaluation prompts/judge versions, baseline adaptation policies, and seeds.

\subsection{Global-Model Safety}
\label{sec:main_results}

Table~\ref{tab:updated_rule_mdjudge} reports the safety of the global language model after each learning stage. At the end of Stage 4, Safe-FCL achieves average Rule and MD-Judge scores of 86.89\% and 90.79\%, respectively, compared with 57.69\% and 56.06\% for FedAvg. These are gains of 29.20 and 34.73 percentage points. Safe-FCL also exceeds FLAME, LASA, Safe-FedLLM-Step, and Safe-FedLLM-Client on both final-stage averages.

Safe-FedLLM-Shadow, however, achieves slightly higher final averages of 87.55\% under Rule and 91.07\% under MD-Judge. Safe-FCL trails Shadow by 0.66 and 0.28 percentage points, respectively. The available results therefore show substantially improved safety over standard and several safety-aware baselines, but do not establish superiority over every compared method.

\subsection{Safety Across Sequential Tasks}
\label{sec:federated_continual_learning}

The lower-triangular results in Table~\ref{tab:updated_rule_mdjudge} also show how safety changes as additional tasks are learned. Safe-FCL attains the highest Rule averages after the first three stages (92.31\%, 92.31\%, and 93.01\%). Under MD-Judge, it ties with Shadow after Stage 1 at 96.04\% and achieves the highest Stage-2 average of 97.32\%; after Stage 3, its average of 94.87\% is slightly below Shadow's 95.34\%.

At the final stage, Safe-FCL's mean Rule score on the three previously learned tasks is 91.06\%, compared with 90.55\% for Shadow. Their corresponding historical-task MD-Judge means are 93.55\% and 93.53\%. In contrast, on the newly learned fourth task, Safe-FCL obtains 74.36\% (Rule) and 82.52\% (MD-Judge), below Shadow's 78.55\% and 83.68\%. Thus, the small final-average gap to Shadow primarily reflects weaker current-task scores, not uniformly worse safety on the earlier tasks.

Historical safety is not perfectly preserved: Safe-FCL's Rule score on Task 3 decreases from 93.47\% immediately after Stage 3 to 86.71\% after Stage 4, while MD-Judge decreases from 95.34\% to 91.14\%. Changes between overall stage averages are not, by themselves, measures of forgetting because each stage average includes a different set of tasks. Moreover, these generation-safety scores should not be conflated with forgetting of benign-task capabilities, which requires a separate utility evaluation.

\subsection{Continual Risk Recognition}
\label{sec:continual_probe_learning}

Table~\ref{tab:safe_fcl_comparison} evaluates the risk detector independently of the generated responses. Safe-FCL achieves AA scores of 99.93\%, 99.99\%, 99.85\%, and 99.64\% across the four stages. After Stage 4, its AA exceeds Safe-FedLLM-Step (79.62\%), Safe-FedLLM-Client (86.25\%), and Safe-FedLLM-Shadow (91.57\%) by 20.02, 13.39, and 8.07 percentage points, respectively.

Safe-FCL's reported AF values are $-0.04$, $0.02$, and $-0.01$ after Stages 2--4, whereas Shadow reports 28.80, 14.55, and 10.55. These results indicate stronger retention of detector-level recognition performance under the reported metric, without implying that every earlier task improves or that the global language model exhibits the same forgetting behavior. Safe-FCL also obtains a New ACC of 99.62\%, compared with 99.48\% for Shadow and 99.60\% for the reported Safe-FCL w/o CRA configuration. The small differences in New ACC contrast with the larger differences in historical-task AA.

The additional Task 5 column currently includes results for Step (93.00\%) and Client (88.33\%), while the corresponding Safe-FCL and Shadow entries are pending. For Safe-FCL, the fifth-stage setting freezes the Stage-4 detector but still trains the global LoRA model on Task 5. Consequently, the available entries do not establish a completed transfer comparison or zero-shot generalization of the global language model.

\subsection{Ablation Study}
\label{sec:ablation_study}

Table~\ref{tab:ablation_avg_t1_t4} compares the available component configurations using the global-model safety scores. Relative to the configuration labeled \emph{w/o Orthogonal + Shadow + Gate}, Safe-FCL raises the Stage-2 Rule and MD-Judge averages from 90.09\% and 96.86\% to 92.31\% and 97.32\%. At Stage 4, the corresponding gains are 0.70 and 0.52 percentage points. These results are consistent with benefits from historical detector protection in the reported settings, although the Stage-3 MD-Judge average is lower for Safe-FCL (94.87\% versus 95.34\%).

Relative to \emph{Orthogonal + Shadow}, Safe-FCL improves the Stage-2 Rule average by 0.35 percentage points while matching its MD-Judge average (97.32\%). At Stage 3, Safe-FCL is lower by 0.08 points under Rule but higher by 0.23 points under MD-Judge. Because the \emph{Orthogonal + Shadow} Stage-4 results are unavailable, the final-stage effect associated with the added module-gating configuration cannot yet be determined.

The probe comparison in Table~\ref{tab:safe_fcl_comparison} provides complementary evidence for CRA. At Stage 2, Safe-FCL improves AA from 98.10\% to 99.99\% over \emph{Safe-FCL w/o CRA}, while AF changes from 3.70 to $-0.04$. At Stage 3, AA improves from 99.71\% to 99.85\%, with AF changing from 0.05 to 0.02. The corresponding Stage-4 ablation entries are still unavailable. Overall, the available comparisons support improved continual risk recognition and competitive safety aggregation, but complete attribution of CRA and FGSA requires the remaining matched results.

